Back to Basics?... or How can supersymmetry be used in simple quantum cosmological model

The general theory of N=1 supergravity with supermatter is applied to a Bianchi type IX diagonal model. The supermatter is constituted by a complex scalar field and its spin-$1\over 2$ fermionic partners. The Lorentz invariant Ansatz for the wave function of the universe, $\Psi$, is taken to be as simple as possible in order to obtain {\it new} solutions. The wave function has a simple form when the potential energy term is set to zero. However, neither the wormhole or the Hartle-Hawking state could be found. The Ansatz for $\Psi$ used in this paper is constrasted with the more general framework of R. Graham and A. Csord\'as.

==> 9505002.tex <==
%Paper: gr-qc/9505002
%From: Paulo Rodrigues Lima Vargas Moniz <P.R.L.V.Moniz@damtp.cam.ac.uk>
%Date: Tue, 2 May 1995 10:49:25 +0100
%Date (revised): Tue, 2 May 1995 11:25:53 +0100

\magnification\magstep0

\openup 1\jot

\input mssymb




\input amssym.def
\input amssym.tex

\def\hbar{\mathchar '26\mkern -9muh}
\font\large=cmbx10 scaled\magstep2

% for text and equations
\catcode`@=11
% at signs act as letters temporarily
\def\eqaltxt#1{\displ@y \tabskip 0pt
  \halign to\displaywidth {%
    \rlap{$##$}\tabskip\centering
    &\hfil$\@lign\displaystyle{##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\tabskip\centering
    &\llap{$\@lign##$}\tabskip\z@skip\crcr
    #1\crcr}}
\def\eqallft#1{\displ@y \tabskip 0pt
  \halign to\displaywidth {%
    $\@lign\displaystyle {##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\crcr
    #1\crcr}}
\catcode`@=12 % at signs are no longer letters

\font\exmafx=msxm10
\font\exmafy=msym10
\def\volm{{\hbox{\exmafy\char'132}}}
\def\vol{{\exmafy\char'132}}
\def\rrr{{\exmafy\char'122}}
\def\rrrm{{\hbox{\exmafy\char'122}}}
\def\cube{{\exmafy\char'003}}
\def\cubem{{\hbox{\exmafy\char'003}}}
\def\nrt{{\exmafy\char'071}}
\def\nrtm{{\hbox{\exmafy\char'071}}}

\def\pound{\hbox{\it \$}}
\def\half{{\textstyle {1 \over 2}}}
\def\third{{\textstyle {1 \over 3}}}
\def\twothirds{{\textstyle {2 \over 3}}}
\def\quarter{{\textstyle {1 \over 4}}}

\def\pmb#1{\setbox0=\hbox{#1}  \kern-.025em\copy0\kern-\wd0
  \kern0.05em\copy0\kern-\wd0  \kern-.025em\raise.0433em\box0 }
\def\pmbh#1{\setbox0=\hbox{#1} \kern-.12em\copy0\kern-\wd0
	    \kern.12em\copy0\kern-\wd0\box0}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt
      \hbox{\vrule width.#2pt height#1pt \kern#1pt
	 \vrule width.#2pt}
      \hrule height.#2pt}}}}

\def\square{{\mathchoice\sqr65\sqr65\sqr54\sqr{3.5}4}\,}

\def\rchi{{\raise 2pt \hbox {$\chi$}}}
\def\rga{{\raise 2pt \hbox {$\gamma$}}}
\def\rg{{\raise 2 pt \hbox {$g$}}}


\def\susy{supersymmetry}
\def\({\left(}
\def\){\right)}
\def\<{\left\langle}
\def\>{\right\rangle}
\def\la{\langle}
\def\ra{\rangle}
\def\lb{\lbrace}
\def\rb{\rbrace}
\def\[{\left[}
\def\]{\right]}
\let\text=\hbox
\def\pt{\partial}
\def\eps{\epsilon}
\def\kap{\kappa}
\def\al{\alpha}
\def\rta{\rightarrow}
\def\lta{\leftarrow}
\def\tr{\triangle}
\def\om{\omega}
\def\ol{\overline}
\def\ul{\underline}
\def\na{\nabla}
\def\inf{\infty}
\def\de{\delta}
\def\lam{\lambda}
\def\ga{\gamma}
\def\ub{\underbar}
\def\Rta{\Rightarrow}
\def\sig{\sigma}
\def\De{\Delta}
\def\ti{\tilde}
\def\cL{{\cal L}}
\def\cC{{\cal C}}
\def\cH{{\cal H}}
\def\cJ{{\cal J}}
\def\cI{{\cal I}}
\def\cD{{\cal D}}
\def\Si{\Sigma}
\def\cl{\centerline}
\def\Lam{\Lambda}
\def\Om{\Omega}
\def\overta{\overrightarrow}
\def\ni{\noindent}
\def\wti{\widetilde}
\def\Ga{\Gamma}
\def\llra{\longleftrightarrow}
\def\what{\widehat}
\def\A{\hbox{$ A\kern -5.5pt / \kern +5.5pt$}}
\def\B{\hbox{$ B\kern -5.5pt / \kern +5.5pt$}}
\def\C{\hbox{$ C\kern -5.5pt / \kern +5.5pt$}}
\def\D{\hbox{$ D\kern -5.5pt / \kern +5.5pt$}}
\def\E{\hbox{$ E\kern -5.5pt / \kern +5.5pt$}}
\def\F{\hbox{$ F\kern -5.5pt / \kern +5.5pt$}}
\def\G{\hbox{$ G\kern -5.5pt / \kern +5.5pt$}}
\def\H{\hbox{$ H\kern -5.5pt / \kern +5.5pt$}}
\def\I{\hbox{$ I\kern -5.5pt / \kern +5.5pt$}}
\def\Z{\hbox{$ Z\kern -5.5pt / \kern +.5pt$}}

\hfuzz 6pt

\catcode`@=12 % at signs are no longer letters
\rightline {\bf DAMTP R95/20}
\font\twelveit=cmti12


\vskip .2 true in
\centerline {\twelveit Back to Basics?$\ldots$}
\centerline {or}
\centerline {\bf How can supersymmetry be used in}
\centerline {\bf a simple quantum cosmological
model\footnote*{\rm Communication
presented at the First Mexican School in Gravitation and Mathematical
Physics, Guanajuato, Mexico, December 12-16, 1994}}
\vskip .1 true in
\centerline {{\rm P.V. Moniz}\footnote{**}{{\rm e-mail address:
prlvm10@amtp.cam.ac.uk}}}
\vskip .1 true in
\centerline {Department of Applied Mathematics and Theoretical Physics}
\centerline{
University of Cambridge}
\centerline{
 Silver Street, Cambridge,
CB3 9EW, UK }
\vskip .2 true in
\centerline {\bf ABSTRACT}
\vskip .1 true in

{\sevenrm The general theory of N=1 supergravity with supermatter is applied
to a Bianchi type IX diagonal model. The supermatter is constituted
by a complex scalar field and its spin-$1\over 2$ fermionic partners.
The Lorentz invariant Ansatz for the wave function of the
universe, $\Psi$,  is taken to be as simple as possible in order to obtain
{\it new} solutions.
The wave function
has a simple form when the  potential energy term
is set to
 zero.  However, neither the
wormhole or the Hartle-Hawking state could be found.
The Ansatz for $\Psi$ used in this paper is constrasted with the more general
framework of
R. Graham and A. Csord\'as.}
\noindent




\magnification\magstep0

\openup 1\jot

\input mssymb
\def\hbar{\mathchar '26\mkern -9muh}
\font\large=cmbx10 scaled\magstep2

% for text and equations
\catcode`@=11
% at signs act as letters temporarily
\def\eqaltxt#1{\displ@y \tabskip 0pt
  \halign to\displaywidth {%
    \rlap{$##$}\tabskip\centering
    &\hfil$\@lign\displaystyle{##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\tabskip\centering
    &\llap{$\@lign##$}\tabskip\z@skip\crcr
    #1\crcr}}
\def\eqallft#1{\displ@y \tabskip 0pt
  \halign to\displaywidth {%
    $\@lign\displaystyle {##}$\tabskip\z@skip
    &$\@lign\displaystyle{{}##}$\hfil\crcr
    #1\crcr}}
\catcode`@=12 % at signs are no longer letters

\font\exmafx=msxm10
\font\exmafy=msym10
\def\volm{{\hbox{\exmafy\char'132}}}
\def\vol{{\exmafy\char'132}}
\def\rrr{{\exmafy\char'122}}
\def\rrrm{{\hbox{\exmafy\char'122}}}
\def\cube{{\exmafy\char'003}}
\def\cubem{{\hbox{\exmafy\char'003}}}
\def\nrt{{\exmafy\char'071}}
\def\nrtm{{\hbox{\exmafy\char'071}}}
\def\pound{\hbox{\it \$}}
\def\half{{\textstyle {1 \over 2}}}
\def\third{{\textstyle {1 \over 3}}}
\def\twothirds{{\textstyle {2 \over 3}}}
\def\quarter{{\textstyle {1 \over 4}}}

\def\pmb#1{\setbox0=\hbox{#1}  \kern-.025em\copy0\kern-\wd0
  \kern0.05em\copy0\kern-\wd0  \kern-.025em\raise.0433em\box0 }

\def\pmbh#1{\setbox0=\hbox{#1} \kern-.12em\copy0\kern-\wd0
	    \kern.12em\copy0\kern-\wd0\box0}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt
      \hbox{\vrule width.#2pt height#1pt \kern#1pt
	 \vrule width.#2pt}
      \hrule height.#2pt}}}}

\def\square{{\mathchoice\sqr65\sqr65\sqr54\sqr{3.5}4}\,}

\def\rchi{{\raise 2pt \hbox {$\chi$}}}
\def\rga{{\raise 2pt \hbox {$\gamma$}}}
\def\rrho{{\raise 2pt \hbox {$\rho$}}}

\def\({\left(}
\def\){\right)}
\def\<{\left\langle}
\def\>{\right\rangle}
\def\la{\langle}
\def\ra{\rangle}
\def\lb{\lbrace}
\def\rb{\rbrace}
\def\[{\left[}
\def\]{\right]}
\let\text=\hbox
\def\pt{\partial}
\def\eps{\epsilon}
\def\kap{\kappa}
\def\al{\alpha}
\def\rta{\rightarrow}
\def\lta{\leftarrow}
\def\tr{\triangle}
\def\om{\omega}
\def\ol{\overline}
\def\ul{\underline}
\def\na{\nabla}
\def\inf{\infty}
\def\de{\delta}
\def\lam{\lambda}
\def\ga{\gamma}
\def\ub{\underbar}
\def\Rta{\Rightarrow}
\def\sig{\sigma}
\def\De{\Delta}
\def\ti{\tilde}
\def\Si{\Sigma}
\def\cl{\centerline}
\def\Lam{\Lambda}
\def\Om{\Omega}
\def\overta{\overrightarrow}
\def\ni{\noindent}
\def\wti{\widetilde}
\def\Ga{\Gamma}
\def\llra{\longleftrightarrow}
\def\what{\widehat}

\def\lrta{\longrightarrow}
\def\cH{{\cal H}}



\medskip


%text start here!%





A quantum gravity theory constitutes a desirable goal in
theoretical physics      as it could lead  to
a proper unification of all know interactions within a
quantum mechanical point of view.
The inclusion of    supersymmetry in
quantum gravity and cosmology allowed  a number
of interesting results and conclusions to be achieved
in the last ten years or so.
Several approaches
may be found  in the literature, namely the triad ADM
canonical formulation,  the $\sigma-$model
supersymmetric extension in quantum cosmology,
and another approach based on Ashtekar variables
(see ref. [1,2] and references therein).

The  canonical quantization framework of N=1 (pure) supergravity was
presented in ref. [3]. It has been pointed out that it
would be sufficient,
in finding a physical state, to solve
the Lorentz and supersymmetry constraints of the theory
  due to the
algebra of constraints of the theory.
The presence of local supersymmetry could also
 contribute  to the removal of divergences.
Moreover,  the supersymmetry constraints
provide a Dirac-like square root of the second order
Wheeler-DeWitt equation. Hence, we were led to solve instead
a set of coupled first-order differential equations
which  $\Psi$ ought to satisfy.


As a result, simple forms for $\Psi$ were obtained,
representing  states such as the
Hartle-Hawking (no-boundary) solution or the (ground state)
wormhole solution [4].
Most of these results seemed then to emphasize a particular basic
track, where   a Dirac-like square-root structure is   used
to obtain directly  any physical states. However,
this {\it back to basics} line\footnote{***}{{\rm  ``Motto'' proposed by  the
current   British Prime Minister some years ago...}} is not the whole story.


On the one hand,
it seemed that the
gravitational and gravitino modes that were allowed to be excited in
 each  supersymmetric Bianchi model contribute in such a way as to
 give only very simple states or even
forbid any physical solutions of the quantum constraints.
Moreover, these states were
found  in the  empty $\psi^0$ (bosonic) and fermionic filled $\psi^6$
sectors and
could be either
wormhole states  or Hartle-Hawking no-boundary states,
according to  different homogeneity conditions for
the gravitino field  (cf. ref. [5]). However, one
could {\it not} find both of them in the same
spectrum of solutions. On the other hand, these solutions in
minisuperspace were shown not to have any counterpart in the
full theory because no states with finite number of
fermions are possible there [6].


These results were then properly interpretated in ref. [7,8],
which  interested readers may wish  to consult.
In fact, the
doubts thereby raised are entire legitemate: even though
canonical quantum supergravity has more constraints
than ordinary quantum gravity, it has surely more
degrees of freedom than gravity.
The cause for the apparent paradoxical results
mentioned in the previous paragraph
was the use
of an Ansatz too special for the $\psi^2$ and $\psi^4$ fermionic
(middle) sectors in the wave function.
This Ansatz [1,2]
allowed only for two bosonic amplitudes
in each of the  middle fermionic sectors and
was constructed only from the Lorentz irreducible
modes of the gravitino field.
There may be   15 such invariants, when we consider
the Lorentz irreducible modes of the gravitational
degrees of freedom as well.
However, these  invariant components correspond now to  a single one
which satisfy a Wheeler-DeWitt type equation. For a particular
factor ordering, we obtain  the wormhole state in the
bosonic sector and the Hartle-Hawking state in the
quartic fermionic sector. Both these states are in the same spectrum
of solutions but this fact has only become possible  by using the
 Wheeler-DeWitt equation.



Hence,  a Dirac-like square-root structure  of gravity with local
supersymmetry could  not directly produce all the desired features
one would like. We still had to
 use a Wheeler-DeWitt equation to obtain the
physical   quantum states altogether in a generic minisuperspace
case. The
(supersymmetric) Dirac-like square roots
seemed not entirely sufficient, even though the
Wheeler-DeWitt type equations (and Hamilton-Jacobi related equations)
used in [7,8]
could be  obtained from the supersymmetry and Lorentz
generators. Nevertheless, the overall picture that appears
could be compared as
 considering  a Dirac equation for a system with
fermionic degres of freedom but that in order to obtain all
physical states in the same spectrum of solutions (cf. ref. [5])
one had to turn to
a Klein-Gordon type-equation. The basic track above mentioned had to be
re-oriented.
But let us also add  the following to the discussion.


The solutions
presented in [7] from the
Wheeler-DeWitt type equation
are  not entirely new in the sense that they can be obtained
 using a specific  definition of
homogeneity conditions for the gravitinos
and  in the context of the
``old'' Ansatz construction [5].
Thus, the ``old'' Ansatz construction could still be usefull
up to a certain point and if properly addressed.

Our objective here is to try to obtain new solutions
from the ``old'' Ansatz construction,
hoping they could bear some  physical significance.
We will
study  a locally supersymmetric
(diagonal) Bianchi type-IX model
coupled to a scalar supermultiplet, formed by
 complex spin-0 scalar fields
together with their
spin-$\half$ partners.
A
 set of first order differential equations obtained
from the supersymmetry constraints will be used , as the ``old''
procedure allows. The obtained  solutions can be expected also to be
 present in the framework  of [7,8]. The results presented here (and in ref.
[9])
may
give  us some insight on how to generalize the approach of [7,8] to
couplings with supermatter.
As we will see, solutions
in the top and bottom sectors as well as in
some middle sectors are obtained for our model when
the  potential is zero
(for more details see [9]). We suspect that these or similar
properties and solutions would also be obtained in the ``new'' approach
but at the expense of having to
deal with  more complicated Wheeler-DeWitt or Hamilton-Jacobi equations.
{\it Of course, we could possibly find out  other solutions
with a more
general Lorentz invariant Ansatz for the wave function of the
universe}.

The Lagrangian of the general theory of N=1 supergravity with supermatter
 is given in eq.~(25.12) of [10] and  it is too long to write out
here. It depends on the tetrad
$ e^{A A'}_{~~~~\mu} $,
 the  spin-${3 \over 2} $
gravitino field $
\( \psi^A_{~~\mu}, \wti \psi^{A'}_{~~\mu} \) $.
on a vector field $ A^{(a)}_\mu $
labelled by a group  index $ (a) $, its  spin-$\half $ partner $ \(
\lam^{(a)}_A, \wti \lam^{(a)}_{A'} \) $, a family of scalars $ \( \Phi^I,
\Phi^{J^*}
\) $ and their  spin-$\half$ partner $ \( \rchi^I_A, \wti \rchi^{J
^*}_{A'} \) $.


 We restrict our case
to a supermatter model constituted only by a scalar field and
its spin$-{1 \over 2}$ partner with a two-dimensional
flat K\"ahler geometry.
The scalar super-multiplet, consisting of a complex massive scalar
field $ \phi $ and spin-$\half$ field $ \rchi, \bar\rchi$
are chosen to be
spatially homogeneous, depending only on time.
The 3-metric
of diagonal Bianchi type-IX
is given by
$ h_{i j} = a_1^2 E^1_{~i} E^1_{~j} + a_2^2 E^2_{~i} E^2_{~j} +
a_3^2 E^3_{~i}
E^3_{~j}~,$
where $ E^j_{~i}$ are
a basis of
left-invariant one-forms on the three-sphere
and $  a_1, a_2, a_3 $ are spatially constant.
We require  the
components
$ \( \psi^A_{~~0}, \ol \psi^{A'}_{~~0} \) $ to
be functions of time only. We
further require that $ \psi^A_{~~i} $ and $ \ti \psi^{A'}_{~~i} $ be
spatially homogeneous in the basis $ e^a_{~i} $.


A quantum description can be made by studying (for example)
Grassmann-algebra-valued wave functions of the form
$ \Psi \[ e^{AA'}_{~~i}, \ \psi^A_{~~i},
\bar \rchi_A, \ \phi,
\ \ol\phi \] $.
The choice of $ \bar \rchi_A \equiv n_A^{~~A'} {\bar \rchi}_{A'} $
rather than $
\rchi_A $ is designed so that the quantum constraint $ \ol S_{A'} $ should
be of first order in momenta




The supersymmetry constraints become then, in differential
operator form
$$ \eqalignno{   \ol S_{A'} &=
 -i\sqrt{2} \[-i \hbar {1\over 4}\[e_{AA'i} \psi^A_j\] e^{CC'i}
{\de \over \de e^{CC'j}}
 -i \hbar {1\over 4}  \[e_{AA'i} \psi^A_j\]   e^{CC'j}
{\de \over \de e^{CC'i}}
 \]
\cr
&
- \sqrt{2} \epsilon^{ijk} e_{AA'i} ~^{3(s)}\om^A_{~~Bj} \psi^B_{~~j}
-{i \over \sqrt{2}}\hbar n_{CA'} \ol \rchi^C {\pt \over \pt \ol \phi}
\cr
&
- i \sqrt{2} \hbar h e^{K/2} P(\phi) n^A_{~~A'} e_{~AB'}^i D^{CB'}_{~~~ji}
{\pt \over \pt \psi^C_j}
- i \sqrt{2} \hbar h e^{K/2} D_\phi P ~ n^A_{~~A'}
{\pt \over \pt \ol \rchi^A}
\cr
&
-{i \over 2\sqrt{2}} h^\half \hbar \phi n^{BB'} n_{CB'}
\ol \rchi^C n_{DA'} \ol \rchi^D { \pt \over \pt \ol \rchi^B}
-{i \over 4\sqrt{2}} \hbar h^\half \phi \epsilon^{ijk}
e^{BB'}_{~~~j} \psi_{kB} D^C_{~~B'li} n_{DA'}\ol\rchi^D
{\pt \over \pt \psi^C_l}
\cr
&
- \hbar \sqrt{2} h^\half
e^{B~~~m}_{~~B'} n^{CB'} \psi_{mC} n_{DA'} \ol \rchi^D
{ \pt \over \pt \ol \rchi^B}
- {i \over \sqrt{2}} \hbar \epsilon^{ijk} e_{AA'j} \psi^A_i
n_{DB'} \ol\rchi^D e^{BB'}_{~~~k}  { \pt \over \pt \ol \rchi^B}
\cr
&
+ {1 \over 2\sqrt{2}} \hbar h^\half \psi_{iA}
(e^{B~~~i}_{~~A'} n^{AC'} - e^{AC'i} n^B_{~~A'})
n_{DC'} \ol \rchi^D { \pt \over \pt \ol \rchi^B},
& (1)\cr}
$$
while the remaining constraint is just the
hermitian conjugate.





The constraints $ J^{A B} \Psi = 0,~~\bar J^{A' B'} \Psi = 0 $
imply that $
\Psi  $ ought to be a Lorentz-invariant function.
Thus, we take   expressions in which all spinor indices have been
contracted together.
It is reasonable also to consider
only wave functions $ \Psi $ which are spatial scalars, i.e.,
 where all spatial
indices $ i, j, \ldots $ have also been contracted together.

We decided to construct our
Lorentz invariant wave function (expressed in several
fermionic sectors and corresponding bosonic amplitudes)
following the view in refs.
[1,2]. We are aware
of its limitations (they may be particularly severe in
the case of $P(\phi)\neq 0$), as far as the middle sectors are
concerned. In fact, we will be neglecting Lorentz
invariants built with not only
the spin $\half$ and $3 \over 2$
Lorentz irreducible mode components of the fermionic fields
but also with the ones corresponding to the
gravitational degrees of freedom.
  We trust, however, that our results
could give some  indication
towards a more complete   implementation.
Our  general Lorentz-invariant wave
function is then taken to be
a polynomial of eight degree in Grassmann variables
$$\eqalignno{\Psi(a_1,a_2,a_3, \phi, \overline{\phi}) &= A +
B_1\beta_A\beta^A + B_2\overline{\chi}_A \overline{\chi}^A
 + C_1 \gamma_{ABC}\gamma^{ABC} \cr
& + D_1 \beta_A\beta^A \gamma_{EBC}\gamma^{EBC}
+ D_2 \overline{\chi}_A \overline{\chi}^A
\gamma_{EBC}\gamma^{EBC}
+ E_1 (\gamma_{ABC}\gamma^{ABC})^2 \cr
&F_1 (\beta_A\beta^A \gamma_{EBC}\gamma^{EBC})^2
+ F_2 \overline{\chi}_A \overline{\chi}^A
(\gamma_{EBC}\gamma^{EBC})^2
+ G_1 \beta_A\beta^A \overline{\chi}_B \overline{\chi}^B \cr & +
H_1 \beta_A\beta^A \overline{\chi}_B
\overline{\chi}^B \gamma_{EDC}\gamma^{EDC}
+ I_1 \beta_A\beta^A \overline{\chi}_B
\overline{\chi}^B (\gamma_{EDC}\gamma^{EDC})^2 \cr
& + Z_1 \overline{\chi}_A\beta^A + Z_2 \overline{\chi}_A\beta^A
\gamma_{EDC}\gamma^{EDC}
 + Z_3 \overline{\chi}_A\beta^A (\gamma_{EDC}\gamma^{EDC})^2~
 &
(2)\cr}$$
The action of the constraints operators
 $S_A, \bar S_{A'}$   on
$\Psi$ lead to a system of coupled first order
differential equations which the bosonic amplitude
coefficients of $\Psi$
ought to satisfy. These coefficients are functions of
$a_1,a_2,a_3,\phi,\bar \phi$.

The  following table illustrate the way the quantum
supersymmetry constraints  operate on $\Psi$
and which types
of fermionic terms can be obtained.
It correspond
to $\ol S_{A'} \Psi$.
A slash over a particular bosonic amplitude
means that after all the calculations have been
made to simplify the corresponding equations, the
expression associated with the particular coefficient
is zero.
A ``$\bullet$'' means that no bosonic
amplitudes in $\Psi$ can match the particular
fermionic
operator.
As a last comment, the third and fourth columns in both
tables correspond to the
action of fermionic operators which appear in terms
involving $P(\phi), D_\phi P(\phi)$ respectively, or their
hermitian conjugates.

\input tables













%TABLE MACRO here%


\begintable
$\searrow$ \| $ \psi$ | $ \ol \chi$ \|
${\pt \over \pt \psi}$ | ${\pt \over \pt \ol\chi}$ \|
$\ol\chi \ol\chi
{\pt \over \pt \ol\chi}$ | $\psi
 \ol \chi
{\pt \over \pt \psi}$
| $\psi \ol\chi
{\pt \over \pt \ol \chi}$
\crthick
$\beta$            \| $A$  | $\bullet$ \| $B_1$  | $Z_1$   \| $\bullet$   |
$\bullet$  | $\bullet$
\cr
$\gamma$           \| $A$  | $\bullet$     \| $\C_1$ | $\bullet$   \| $\bullet$
   | $\bullet$ | $\bullet$
\cr
$\ol\chi$          \| $\bullet$  | $A$ \| $Z_1$    |  $B_2$\| $\bullet$ |
$\bullet$     | $\bullet$
\cr
$\beta\beta\ol\chi$\| $Z_1$   | $B_1$ \| $\bullet$ |$G_1$ \| $\bullet$    |
$B_1$     | $Z_1$
\cr
$\beta\beta\gamma$ \| $B_1$  | $\bullet$     \| $\D_1$| $\bullet$   \|
$\bullet$    | $\bullet$ | $\bullet$
\cr
$\beta\ol\chi
\ol\chi$           \| $B_2$  | $Z_1$ \| $G_1$| $\bullet$\| $Z_1$   | $Z_1$ |
$B_2$
\cr
$\beta\ol\chi
\gamma$            \| $Z_1$  | $\bullet$     \| $\bullet$    | $\bullet$   \|
$\bullet$    |$C_1,B_1$| $Z_1$
\cr
 $\beta\gamma\gamma$\| $C_1$  | $\bullet$ \| $D_1$| $Z_2$   \| $\bullet$    |
$\bullet$  | $\bullet$
\cr
$\ol\chi\ol\chi
\gamma$            \| $B_2$  | $\bullet$     \|$\D_2$| $\bullet$   \| $\bullet$
   | $\Z_1$     |$\B_2$
\cr
$\ol\chi\gamma
\gamma$             \| $\bullet$  | $G_1$  \| $Z_2$    |  $B_2$ \| $\bullet$ |
$C_1$  | $\bullet$
\cr
$\gamma\gamma
\gamma$            \|$C_1$   |  $\bullet$    \|$\E_1$| $\bullet$   \| $\bullet$
   |$\bullet$ |   $\bullet$
\cr
$\beta(\gamma
\gamma)^2$          \|$E_1$   | $\bullet$  \| $F_1$| $Z_3$   \| $\bullet$    |
$\bullet$ | $\bullet$
\cr
$\gamma\beta\beta
\gamma\gamma$      \|$D_1$   |$\bullet$      \|$\F_1$|  $\bullet$  \| $\bullet$
   | $\bullet$ |$\bullet$
\cr
$\gamma\ol\chi\ol
\chi\gamma
\gamma $           \|$D_2$   | $\bullet$     \|$\F_2$| $\bullet$   \| $\bullet$
   | $Z_2$   | $\D_2$
\cr
$\beta\ol\chi
\ol\chi
\gamma\gamma$     \|$D_2$    |$Z_2$ \| $H_1$ |$\bullet$ \|  $Z_2$   | $Z_2$
|$D_2$
\cr
$\gamma\beta
\beta\ol\chi
\ol\chi$          \|$G_1$    |  $\bullet$   \|$\H_1$ |$\bullet$   \|  $\bullet$
   | $Z_2$  |$\H_1$
\cr
$\ol\chi
(\gamma\gamma)^2$ \| $\bullet$    | $E_1$ \| $Z_3$ | $F_2$ \|  $\bullet$
|$E_1$|  $\bullet$
\cr
$\ol\chi
\beta\gamma
\gamma\gamma$     \|$Z_2$    |  $\bullet$   \| $\bullet$    |  $\bullet$  \|
$\bullet$    |$D_1,E_1$|$Z_2$
\cr
$\ol\chi\beta
\beta\gamma
\gamma$           \|  $Z_2$      | $D_1$\| $\bullet$    | $H_1$ \| $\bullet$ |
$D_1$| $Z_2$
\cr
$\beta\ol\chi\ol
\chi\(\gamma
\gamma\)^2$        \| $F_2$   | $Z_3$\|$I_1$ | $\bullet$ \|  $Z_3$  | $Z_3$
|$F_2$
\cr
$\gamma
\beta\beta
\ol\chi
\ol\chi
\gamma\gamma$     \| $H_1$   |  $\bullet$   \|$\I_1$ | $\bullet$  \|
$\bullet$   |  $\bullet$   |$\H_1$
\cr
$\ol\chi\beta
\beta(\gamma
\gamma)^2$        \| $Z_3$       | $F_1$\| $\bullet$    |$I_1$\| $\bullet$
| $F_1$|$Z_3$
\endtable




\centerline{{\bf Table 1}: Action of $\ol S_{A'}$  on $\Psi$ }

We then analysed two possible cases, namely when  the
scalar field dependent  potential
in the supermatter content was either arbitrary
or identically set to zero.
In the
former, our main (and perhaps, solely) conclusion
was that the adequacy of our Ansatz for $\Psi$ is
severly limited.
The constraints
imply $\Psi = 0$ for some simplifying assumptions.
In a more general setting, no easy way is apparent of
obtaining an analytical solution for the full set of equations.
In fact, exponential terms as $e^{\phi\ol\phi}$ lead to
serious difficulties.

In the latter, however, we found out that $\Psi$ had indeed
a very simple form.
More precisely, we obtained
$$\eqalignno{ \Psi &=
  f(\overline{\phi}) e^{[-a_1^2 - a_2^2 - a_3^2]}
+
 h(\phi) a_1a_2a_3 e^{[-a_1^2
- a_2^2 - a_3^2]} e^{-2\pi^2 \phi
\overline{\phi}}
 \overline{\chi}_A\overline{\chi}^A \cr
&
+
 g(\ol\phi) a_1a_2a_3 e^{[a_1^2 + a_2^2  + a_3^2]}
e^{-2\pi^2\phi
\overline{\phi}}
\beta_A\beta^A(\gamma_{BCD}\gamma^{BCD})^2 +
 k(\phi)  e^{[a_1^2 + a_2^2 + a_3^2]}
\overline{\chi}_A\overline{\chi}^A\beta_E\beta^E(\gamma_{BCD}\gamma^{BCD})^2.
& (3) \cr} $$
Unfortunately, we cannot find the
Hartle-Hawking and wormhole
states
in eq.(3) [9].


It seems though from our analysis and discussion hereby
presented that when supermatter is present, one cannot
simply expect to follow a somewhat simple relation
between the old and new frameworks. Perhaps the approach
in [7,8] properly applied to our Bianchi-IX model could
be able to find out the
Hartle-Hawking states in {\it other} middle sectors.
However, the absence of a wormhole state is another
issue to be properly addressed [10].
Overall, we hope our results
(see ref. [9] as well) could provide  new ground for a debate
on supersymmetric quantum cosmology with supermatter fields.






\medskip



\noindent
{\bf ACKNOWLEDGEMENTS}

The author is  thankful to R. Caldwell for assistance with TeX macros,
to A.D.Y. Cheng for many  discussions
and for sharing his points of view and to
S.W. Hawking for helpful
  conversations.
Discussions with  O. Obregon and R. Graham are also acnowledged.
The author   gratefully acknowledges
the Instituto de Fisica de la Universidad de Guanajuato, Mexico,
for supporting part of his 3 weeks visit
as well as
the support of
a Human Capital and Mobility (HCM)
Fellowship from the European Union (Contract ERBCHBICT930781).

\medskip


\noindent
{\bf REFERENCES}

{\rm

\advance\leftskip by 4em
\parindent = -4em

[1]  A.D.Y. Cheng, P.D. D'Eath and
P.R.L.V. Moniz,
{\it Proc. - Gravitation and Cosmology}
{\bf 1} (1995) 1



[2]  A.D.Y. Cheng, P.D. D'Eath and
P.R.L.V. Moniz,
{\it Proc. - Gravitation and Cosmology}
{\bf 1} (1995) 12




[3] P.D. D'Eath, Phys.~Rev.~D {\bf 29}, 2199 (1984).


[4] S.W. Hawking and D.N. Page, Phys.~Rev.~D {\bf 42}, 2655 (1990);
J.B. Hartle and S.W. Hawking, Phys.~Rev.~D {\bf 28}, 2960 (1983).




[5] R. Graham and H. Luckock, Phys. Rev. D
{\bf 49}, R4981 (1994).



[6] S. Carroll, D. Freedman, M. Ortiz and
D. Page, Nuc. Phys. B{\bf 423}, 3405 (1994).


[7] R. Graham and A. Csord\'as, {\it
Nontrivial fermion states in supersymmetric minisuperspace},
in:
Proceedings of the First Mexican School in Gravitation
and Mathematical Physics,
Guanajuato, Mexico,  December 12-16, 1994.

[8]  R. Graham and A. Csord\'as, {\it
Supersymmetric minisuperspace with non-vanishing fermion number},
gr-qc 9502004.


[9]  P.V. Moniz, {\it Quantization of the Bianchi type-IX
model in N=1  Supergravity in the
Presence of Supermatter}, DAMTP report R95/21.

[10] P.V. Moniz, {\it Is there a Problem
with Quantum Wormholes in N=1 Supergravity?}, DAMTP R95/19



\ \ \ }


\bye


%Macro for tables start here. Just copy it %
%to a file named ``tables.tex'' and put it into your directory%


% Received from Jnet%SLACVM::SHARON  1-MAR-1988 13:16
% Subj:	TABLES TEX
% +--------------------------------------------------------------------+
% |                                                                    |
% |                           TABLES.TEX                               |
% |                                                                    |
% |                     Ray F. Cowan  15-Feb-85                        |
% |                                                                    |
% |                       Princeton University                         |
% |                                                                    |
% |                     Last Revision: 17-Apr-86                       |
% |                                                                    |
% |   Macros I find handy for making tables.  See TABLEDOC TEX for     |
% |   a longer description.  The token-counting macros are straight    |
% |   from the TeXbook's "Dirty Tricks" appendix.                      |
% |                                                                    |
% +--------------------------------------------------------------------+
%
%AJS3 renamed "\header" macro to "\headertab" to avoid interference with other
%     "\header" macros.
%
\newbox\hdbox%
\newcount\hdrows%
\newcount\multispancount%
\newcount\ncase%
\newcount\ncols% This is the number of primary text columns in the table.
\newcount\nrows%
\newcount\nspan%
\newcount\ntemp%
\newdimen\hdsize%
\newdimen\newhdsize%
\newdimen\parasize%
\newdimen\spreadwidth%
\newdimen\thicksize%
\newdimen\thinsize%
\newdimen\tablewidth%
\newif\ifcentertables%
\newif\ifendsize%
\newif\iffirstrow%
\newif\iftableinfo%
\newtoks\dbt%
\newtoks\hdtks%
\newtoks\savetks%
\newtoks\tableLETtokens%
\newtoks\tabletokens%
\newtoks\widthspec%
%
%  Book-keeping stuff--see how often these macros are called.
%
\immediate\write15{%
CP SMSG GJMSINK TEXTABLE --> TABLE MACROS V. 851121 JOB = \jobname%
}%
%
%  Turn on table diagnostics.
%
\tableinfotrue%
\catcode`\@=11%  Allows use of "@" in macro names, like PLAIN.TEX does.
\def\out#1{\immediate\write16{#1}}%  Debugging aid.  Writes #1 on the
%                                    user's terminal and in the log file.
%
%  Define the \tstrut height, depth in terms of the x_height parameter.
%
\def\tstrut{\vrule height3.1ex depth1.2ex width0pt}%
\def\and{\char`\&}%  Allows us to get an `&' in the text.  This is the
%                    same as using the PLAIN TeX macro \&.
\def\tablerule{\noalign{\hrule height\thinsize depth0pt}}%
\thicksize=1.5pt%  Default thickness for fat rules.  The user should feel
%                  free to change this to his preference.
\thinsize=0.6pt%   Default thickness for thin rules.
\def\thickrule{\noalign{\hrule height\thicksize depth0pt}}%
\def\hrulefill{\leaders\hrule\hfill}%
\def\bigrulefill{\leaders\hrule height\thicksize depth0pt \hfill}%
\def\ctr#1{\hfil\ #1\hfil}%
\def\altctr#1{\hfil #1\hfil}%
\def\vctr#1{\hfil\vbox to0pt{\vss\hbox{#1}\vss}\hfil}%
%
%  Here are things for controlling the width of the finished table.
%
\tablewidth=-\maxdimen%
\spreadwidth=-\maxdimen%
\def\tabskipglue{0pt plus 1fil minus 1fil}%
%
%  Stuff for centering or not.
%
\centertablestrue%
\def\centeredtables{%
   \centertablestrue%
}%
\def\noncenteredtables{%
   \centertablesfalse%
}%
%
%  \vctr vertically centers its argument in the row.
%
\parasize=4in%
\long\def\para#1{%  Used to make little paragraphs out of one entry.
   {%
      \vtop{%
         \hsize=\parasize%
         \baselineskip14pt%
         \lineskip1pt%
         \lineskiplimit1pt%
         \noindent #1%
         \vrule width0pt depth6pt%
      }%
   }%
}%
%
\gdef\ARGS{########}%  Produces the correct number of #'s in the preamble
%                      by the time eveything is expanded and \halign sees
%                      it.
\gdef\headerARGS{####}%  Same as \ARGS, but used in \headertab macros.
\def\@mpersand{&}%  Allows us to get alignment tab characters later
%                   when we have made the character "&" an active macro.
{\catcode`\|=13%  Make |'s locally active.
\gdef\letbarzero{\let|0}%  Globally define a macro that allows us to
%                          keep active |'s from being expanded in edef's.
\gdef\letbartab{\def|{&&}}%
\gdef\letvbbar{\let\vb|}%
%  This \def will cause active |'s read by
%                            \ruledtable to be converted into double
%                            alignment tabs.
}%  End of locally active |'s.
%
{\catcode`\&=4%  Make these alignment tabs.
\def\ampskip{&\omit\hfil&}%  This local macro skips a vertical rule.
\catcode`\&=13%  Now make &'s into active macros.
\let&0%  This allows us to expand \ampskip in the next \xdef without
%        attempting to expand the & and getting an "undefined control
%        sequence" error.
\xdef\letampskip{\def&{\ampskip}}%
\gdef\letnovbamp{\let\novb&\let\tab&}
%  This will cause active &'s read by
%                                   \ruledtable to be converted into
%                                   double tabs and an \omit'ted \vrule.
}%  End of locally active &'s.
%
\def\begintable{%  Here we make |'s and &'s active characters so we can
%                  interpret them as macros.  Note that this action is
%                  true only until we encounter the matching \endgroup
%                  token later at the end of the \ruledtable macro.
   \begingroup%
   \catcode`\|=13\letbartab\letvbbar%
   \catcode`\&=13\letampskip\letnovbamp%
   \def\multispan##1{%  We must redefine \multispan to count the number
%                       of primary columns, not physical columns.
      \omit \mscount##1%
      \multiply\mscount\tw@\advance\mscount\m@ne%
      \loop\ifnum\mscount>\@ne \sp@n\repeat%
   }%  End of \multispan macro.
   \def\|{%
      &\omit\widevline&%
   }%
   \ruledtable%  Now we call \ruledtable to do the real work.
}%  End of \begintable macro.
%
\long\def\ruledtable#1\endtable{%
%
%  This macro reads in the user's data entries
%  and converts them into a ruled table.
%
%  Important note:  Many macros and parameters are re-defined here, and
%  these must be kept local to the table macros to avoid conflict with
%  their use outside of tables.  This is done by the \begingroup token
%  macro \begintable and the \endgroup token at the end of
%  this macro.
%
   \offinterlineskip%  Needed to make rules touch each other.
   \tabskip 0pt%  Needed for same reason as \offinterlineskip.
   \def\widevline{\vrule width\thicksize}%  Make outer \vrule's wider.
   \def\endrow{\@mpersand\omit\hfil\crnorm\@mpersand}%
   \def\crthick{\@mpersand\crnorm\thickrule\@mpersand}%
   \def\crthickneg##1{\@mpersand\crnorm\thickrule
          \noalign{{\skip0=##1\vskip-\skip0}}\@mpersand}%
   \def\crnorule{\@mpersand\crnorm\@mpersand}%
   \def\crnoruleneg##1{\@mpersand\crnorm
          \noalign{{\skip0=##1\vskip-\skip0}}\@mpersand}%
   \let\nr=\crnorule%  A shorter abbreviation.
   \def\endtable{\@mpersand\crnorm\thickrule}%
%
   \let\crnorm=\cr%  Allows us to use \cr for our own purposes.
%
%  Cause user-typed \cr's to follow a row with a \tablerule.
%
   \edef\cr{\@mpersand\crnorm\tablerule\@mpersand}%
   \def\crneg##1{\@mpersand\crnorm\tablerule
          \noalign{{\skip0=##1\vskip-\skip0}}\@mpersand}%
   \let\ctneg=\crthickneg
   \let\nrneg=\crnoruleneg
%
   \the\tableLETtokens%  Get the user's extra \let's, if any.
%
%  Put the data entries into a token register so we can scan through them
%  and see what the user is asking us to do.
%
   \tabletokens={&#1}%  We add an extra alignment tab to the beginning
%                       of the first row to allow for the first \vrule.
%
%  Now count how many rows are in the table and return the result in
%  count register \nrows; do the same for columns, and return that
%  in register \ncols.
%
   \countROWS\tabletokens\into\nrows%
   \countCOLS\tabletokens\into\ncols%
%
%  Now do a little arithmetic to convert the number of primary columns
%  into the number of physical columns that the alignment preamble must
%  prepare for;  similarly for rows.
%
   \advance\ncols by -1%
   \divide\ncols by 2%
   \advance\nrows by 1%
%
%  Tell the user how many rows and columns we found in his data, if he
%  wants to know.
%
   \iftableinfo %
      \immediate\write16{[Nrows=\the\nrows, Ncols=\the\ncols]}%
   \fi%
%
%  Now we actually go ahead and produce the table.
%
   \ifcentertables
      \ifhmode \par\fi%  Make sure we are in vertical mode.
      \line{%  The final table comes out as an \hbox of width the \hsize.
      \hss%  The final table will be centered left-to-right.
   \else %
      \hbox{%
   \fi
      \vbox{%
         \makePREAMBLE{\the\ncols}%  Generate the preamble.
         \edef\next{\preamble}%  This line and the next line force the
         \let\preamble=\next%    expansion of all \ARGS tokens into the
%                                appropriate number of #'s.
         \makeTABLE{\preamble}{\tabletokens}%  Go do the \halign here.
      }%  End of \vbox.
      \ifcentertables \hss}\else }\fi%  Finish the centering effect.
%                                       It is important that no spaces
%                                       follow the two `}' here.
%  }%  End of \line.
   \endgroup%  Return all local macros and parameters to their outside
%              values.
   \tablewidth=-\maxdimen%  Reset \tablewidth to normal.
   \spreadwidth=-\maxdimen% Same for \spreadwidth.
}%  End of macro \ruledtable.
%
\def\makeTABLE#1#2{%  Does an \halign for the \ruledtable macro.
   {%  Start of local parameter values.
%
   \let\ifmath0%     These macros would cause trouble if they were to be
   \let\headertab0%  expanded in the following \xdef; we \let them be
   \let\multispan0%  equal to a digit, because digits can't be expanded.
%
%  Set up the width specification here.
%
   \ncase=0%
   \ifdim\tablewidth>-\maxdimen \ncase=1\fi%
   \ifdim\spreadwidth>-\maxdimen \ncase=2\fi%
   \relax%  This \relax is absolutely necessary, without it the following
%           \ifcase will always take \ncase=0.
%
   \ifcase\ncase %
      \widthspec={}%
   \or %
      \widthspec=\expandafter{\expandafter t\expandafter o%
                 \the\tablewidth}%
   \else %
      \widthspec=\expandafter{\expandafter s\expandafter p\expandafter r%
                 \expandafter e\expandafter a\expandafter d%
                 \the\spreadwidth}%
   \fi %
%\out{Widthspec=[\the\widthspec]}%
%\out{Preamble=[\preamble]}%
   \xdef\next{%  We must force the preamble to be expanded BEFORE the
      \halign\the\widthspec{%
%        \halign is done;  this \edef\next{...}\next construction
%                does the trick.
      #1%  This is the preamble text.
%
      \noalign{\hrule height\thicksize depth0pt}%  Makes the top \hrule.
%
      \the#2\endtable%  This is the main body.
%
%     \noalign{\hrule height0.7pt depth0pt}%  Makes the last \hrule.
      }%  End of \halign.
   }%  End of \next.
   }%  End of local values.
   \next%  This \next must be outside of the local values, because now
%          we want those troublesome macros in the \let's above to have
%          their normal actions.
}%  End of macro \makeTABLE.
%
\def\makePREAMBLE#1{%  This macro generates the necessary preamble for a
%                      ruled table with #1 primary columns.
%                      (Primary columns means the number of columns NOT
%                       counting those used for vertical rules.)
   \ncols=#1%  Get the number of columns desired.
   \begingroup%  Start local parameter definitions.
   \let\ARGS=0%  This is the key to the whole thing; it prevents \ARGS
%                from being expanded in the following \edef's.
   \edef\xtp{\widevline\ARGS\tabskip\tabskipglue%
   &\ctr{\ARGS}\tstrut}%  A 1-column preamble.  Gets the sizing right.
   \advance\ncols by -1%  One column has been generated; decrement the
%                         counter.
   \loop%  Append as many further columns as needed to the preamble.
      \ifnum\ncols>0 %
      \advance\ncols by -1%
      \edef\xtp{\xtp&\vrule width\thinsize\ARGS&\ctr{\ARGS}}%
   \repeat
   \xdef\preamble{\xtp&\widevline\ARGS\tabskip0pt%
   \crnorm}%  Adds the last \vrule.
   \endgroup%  End of local parameters.
}%  End of macro \makePREAMBLE.
%
\def\countROWS#1\into#2{%  This counts the number of rows in #1 by
%                          looking for control sequences that end a row,
%                          e.g., \cr, \crthick, etc., and puts the result
%                          into count register #2.
   \let\countREGISTER=#2%
   \countREGISTER=0%
%  \out{In countROWS:  tokens are [\the#1]}%
   \expandafter\ROWcount\the#1\endcount%
}%
%
\def\ROWcount{%
   \afterassignment\subROWcount\let\next= %
}%
\def\subROWcount{%
%  \out{In subROWcount:  next is [\meaning\next]}%  Debugging aid.
   \ifx\next\endcount %
      \let\next=\relax%
   \else%
      \ncase=0%
      \ifx\next\cr %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\endrow %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crthick %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crnorule %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crthickneg %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crnoruleneg %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crneg %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\headertab %
%     \out{In subROWcount:  next=header, ncase set=1}%
         \ncase=1%
      \fi%
%     \out{In subROWcount:  ncase is [\the\ncase]}%
      \relax%
      \ifcase\ncase %
         \let\next\ROWcount%
%        \out{subROWcount---> ncase=\the\ncase}%
      \or %
         \let\next\argROWskip%
%        \out{subROWcount---> ncase=\the\ncase}%
      \else %
      \fi%
   \fi%
%  \out{subROWcount---> NEXT=\meaning\next}%
   \next%
}%  End of macro \subROWcount.
%
\def\counthdROWS#1\into#2{%
\dvr{10}%
   \let\countREGISTER=#2%
   \countREGISTER=0%
\dvr{11}%
%  \out{In counthdROWS:  tokens are [\the#1]}%
\dvr{13}%
   \expandafter\hdROWcount\the#1\endcount%
\dvr{12}%
}%
%
\def\hdROWcount{%
   \afterassignment\subhdROWcount\let\next= %
}%
\def\subhdROWcount{%
%\out{In subhdROWcount:  next is [\meaning\next]}%
   \ifx\next\endcount %
      \let\next=\relax%
   \else%
      \ncase=0%
      \ifx\next\cr %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\endrow %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crthick %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\crnorule %
         \global\advance\countREGISTER by 1%
         \ncase=0%
      \fi%
      \ifx\next\headertab %
%\out{In subhdROWcount:  next=header, ncase set=1}%
         \ncase=1%
      \fi%
%\out{In subhdROWcount:  ncase is [\the\ncase]}%
\relax%
      \ifcase\ncase %
         \let\next\hdROWcount%
%\out{subhdROWcount---> ncase=\the\ncase}%
      \or%
         \let\next\arghdROWskip%
%\out{subhdROWcount---> ncase=\the\ncase}%
      \else %
      \fi%
   \fi%
%\out{subhdROWcount---> NEXT=\meaning\next}%
   \next%
}%
%
{\catcode`\|=13\letbartab
\gdef\countCOLS#1\into#2{%
%  \out{In countCOLS:  tokens are [\the#1]}
   \let\countREGISTER=#2%
   \global\countREGISTER=0%
   \global\multispancount=0%
   \global\firstrowtrue
   \expandafter\COLcount\the#1\endcount%
   \global\advance\countREGISTER by 3%
   \global\advance\countREGISTER by -\multispancount
%  \out{countCOLS-->[\the\countREGISTER]}
}%
%
\gdef\COLcount{%
   \afterassignment\subCOLcount\let\next= %
}%
{\catcode`\&=13%
\gdef\subCOLcount{%
%\out{In subCOLcount: next is [\meaning\next]}
   \ifx\next\endcount %
      \let\next=\relax%
   \else%
      \ncase=0%
      \iffirstrow
         \ifx\next& %
            \global\advance\countREGISTER by 2%
            \ncase=0%
         \fi%
         \ifx\next\span %
            \global\advance\countREGISTER by 1%
            \ncase=0%
         \fi%
         \ifx\next| %
            \global\advance\countREGISTER by 2%
            \ncase=0%
         \fi
         \ifx\next\|
            \global\advance\countREGISTER by 2%
            \ncase=0%
         \fi
         \ifx\next\multispan
            \ncase=1%
            \global\advance\multispancount by 1%
         \fi
         \ifx\next\headertab
            \ncase=2%
         \fi
         \ifx\next\cr       \global\firstrowfalse \fi
         \ifx\next\endrow   \global\firstrowfalse \fi
         \ifx\next\crthick  \global\firstrowfalse \fi
         \ifx\next\crnorule \global\firstrowfalse \fi
         \ifx\next\crnoruleneg \global\firstrowfalse \fi
         \ifx\next\crthickneg  \global\firstrowfalse \fi
         \ifx\next\crneg       \global\firstrowfalse \fi
      \fi%  End of \iffirstrow.
\relax%\out{subCOL-->  ncase=[\the\ncase]}
% \out{subCOL-->  next=\meaning\next}
      \ifcase\ncase %
         \let\next\COLcount%
      \or %
         \let\next\spancount%
      \or %
         \let\next\argCOLskip%
      \else %
      \fi %
   \fi%
%  \out{subCOL-->  countREGISTER=[\the\countREGISTER]}
   \next%
}%
\gdef\argROWskip#1{%
%  Deletes the next balanced, undelimited argument from a
%                 token list.
% \out{---> Entering argROWskip <---}
% \out{In argROWskip:  deleted arg is [#1]}%
   \let\next\ROWcount \next%
}%  End of macro \argskip.
\gdef\arghdROWskip#1{%
%  Deletes the next balanced, undelimited argument from a
%                 token list.
% \out{---> Entering arghdROWskip <---}
% \out{In arghdROWskip:  deleted arg is [#1]}%
   \let\next\ROWcount \next%
}%  End of macro \arghdROWskip.
\gdef\argCOLskip#1{%
%  Deletes the next balanced, undelimited argument from a
%                 token list.
% \out{---> Entering argCOLskip <---}
% \out{In argCOLskip:  deleted arg is [#1]}%
   \let\next\COLcount \next%
}%  End of macro \argskip.
}%  End of active &'s.
}%  End of active |'s.
\def\spancount#1{%\out{spancount--->\meaning#1}
   \nspan=#1\multiply\nspan by 2\advance\nspan by -1%
   \global\advance \countREGISTER by \nspan
%  \out{number spancount--->\the\nspan; \the\countREGISTER}
   \let\next\COLcount \next}%
%
%\def\dvr#1{\vrule width 1.0pt depth 0pt height 12pt$_{#1}$}
\def\dvr#1{\relax}%
% \omit\hfil%
% \parindent=0pt\hsize=1.1in\valign{%
% \vfil#\vfil&\vfil#\vfil\cr\hfil\hbox{\ Added to\ }\hfil&%
% \hfil\hbox{\ empty events\ }\hfil\cr}\hfil%
\def\headertab#1{%
\dvr{1}{\let\cr=\@mpersand%
\hdtks={#1}%
%\out{In header:  hdtks=[\the\hdtks]}%
\counthdROWS\hdtks\into\hdrows%
\advance\hdrows by 1%
\ifnum\hdrows=0 \hdrows=1 \fi%
%\out{In header:  Nhdrows=[\the\hdrows]}%
\dvr{5}\makehdPREAMBLE{\the\hdrows}%
%\out{In header:  headerpreamble=[\headerpreamble]}%
\dvr{6}\getHDdimen{#1}%
%\out{In header:  hdsize=[\the\hdsize]}%
%\striplastCR{#1}%
{\parindent=0pt\hsize=\hdsize{\let\ifmath0%
\xdef\next{\valign{\headerpreamble #1\crnorm}}}\dvr{7}\next\dvr{8}%
}%
}\dvr{2}}%  End of macro \headertab.
%\def\striplastCR#1\cr{\xdef\headerbody{#1}}%
\def\makehdPREAMBLE#1{%This macro generates the necessary preamble for a
\dvr{3}%
%                      ruled table with \ncols primary columns.
%                      (Primary columns means the number of columns NOT
%                       counting those used for vertical rules.
\hdrows=#1%  Get the number of columns desired.
{%  Start local parameter definitions.
\let\headerARGS=0%
%  This is the key to the whole thing; it prevents \ARGS
\let\cr=\crnorm%
%                from being expanded in the followin \edef's.
\edef\xtp{\vfil\hfil\hbox{\headerARGS}\hfil\vfil}%
\advance\hdrows by -1%  One row has been generated; decrement the
%                         counter.
\loop%  Append as many further rows as needed to the preamble.
\ifnum\hdrows>0%
\advance\hdrows by -1%
\edef\xtp{\xtp&\vfil\hfil\hbox{\headerARGS}\hfil\vfil}%
\repeat%
\xdef\headerpreamble{\xtp\crcr}%
}%  End of local parameters.
\dvr{4}}%  End of \makehdPREAMBLE.
%
\def\getHDdimen#1{%
%\out{In getHDdimen:  Arg 1=[#1]}%
\hdsize=0pt%
\getsize#1\cr\end\cr%
}%  End of macro getHDdimen.
\def\getsize#1\cr{%
%\out{In getsize:  Arg 1=[#1]}%
%  Here we have to check arg#1 and see if the first token in #1 is an
%    \end; if so, we stop, else we check the width of arg#1.
%  We recall that each arg#1 will be terminated with a \cr token.
\endsizefalse\savetks={#1}%
%\out{In getsize:  the savetks = [\the\savetks]}%
\expandafter\lookend\the\savetks\cr%
%\out{In getsize:  ifendsize = [\meaning\ifendsize]}%
\relax \ifendsize \let\next\relax \else%
\setbox\hdbox=\hbox{#1}\newhdsize=1.0\wd\hdbox%
\ifdim\newhdsize>\hdsize \hdsize=\newhdsize \fi%
%\out{In getsize:  hdsize=[\the\hdsize]}%
%\out{In getsize:  newhdsize=[\the\newhdsize]}%
\let\next\getsize \fi%
\next%
}%
\def\lookend{\afterassignment\sublookend\let\looknext= }%
\def\sublookend{\relax%
%\out{In sublookend:  looknext = [\looknext]}%
\ifx\looknext\cr %
%\out{In sublooknext:  looknext=cr}%
\let\looknext\relax \else %
%\out{In sublooknext:  looknext/=cr}%
   \relax
   \ifx\looknext\end \global\endsizetrue \fi%
   \let\looknext=\lookend%
    \fi \looknext%
}%
%
%  Allow the user to make his own names for crthick, etc.
%
\def\tablelet#1{%
   \tableLETtokens=\expandafter{\the\tableLETtokens #1}%
}%
\catcode`\@=12%  Change @'s back to their normal category code.
%






==> mssymb.tex <==
%		*****	  MSSYMB.TeX	*****		       8 Jul 87
%
%	This file contains the definitions for the symbols in the two
%	"extra symbols" fonts created at the American Math. Society.

\catcode`\@=11

\font\tenmsx=msxm10
\font\sevenmsx=msxm7
\font\fivemsx=msxm5
\font\tenmsy=msym10
\font\sevenmsy=msym7
\font\fivemsy=msym5
\newfam\msxfam
\newfam\msyfam
\textfont\msxfam=\tenmsx  \scriptfont\msxfam=\sevenmsx
  \scriptscriptfont\msxfam=\fivemsx
\textfont\msyfam=\tenmsy  \scriptfont\msyfam=\sevenmsy
  \scriptscriptfont\msyfam=\fivemsy

\def\hexnumber@#1{\ifcase#1 0\or1\or2\or3\or4\or5\or6\or7\or8\or9\or
	A\or B\or C\or D\or E\or F\fi }

%  The following 13 lines establish the use of the Euler Fraktur font.
%  To use this font, remove % from beginning of these lines.
%\font\teneuf=eufm10
%\font\seveneuf=eufm7
%\font\fiveeuf=eufm5
%\newfam\euffam
%\textfont\euffam=\teneuf
%\scriptfont\euffam=\seveneuf
%\scriptscriptfont\euffam=\fiveeuf
%\def\frak{\relaxnext@\ifmmode\let\next\frak@\else
% \def\next{\Err@{Use \string\frak\space only in math mode}}\fi\next}
%\def\goth{\relaxnext@\ifmmode\let\next\frak@\else
% \def\next{\Err@{Use \string\goth\space only in math mode}}\fi\next}
%\def\frak@#1{{\frak@@{#1}}}
%\def\frak@@#1{\noaccents@\fam\euffam#1}
%  End definition of Euler Fraktur font.

\edef\msx@{\hexnumber@\msxfam}
\edef\msy@{\hexnumber@\msyfam}

\mathchardef\boxdot="2\msx@00
\mathchardef\boxplus="2\msx@01
\mathchardef\boxtimes="2\msx@02
\mathchardef\square="0\msx@03
\mathchardef\blacksquare="0\msx@04
\mathchardef\centerdot="2\msx@05
\mathchardef\lozenge="0\msx@06
\mathchardef\blacklozenge="0\msx@07
\mathchardef\circlearrowright="3\msx@08
\mathchardef\circlearrowleft="3\msx@09
\mathchardef\rightleftharpoons="3\msx@0A
\mathchardef\leftrightharpoons="3\msx@0B
\mathchardef\boxminus="2\msx@0C
\mathchardef\Vdash="3\msx@0D
\mathchardef\Vvdash="3\msx@0E
\mathchardef\vDash="3\msx@0F
\mathchardef\twoheadrightarrow="3\msx@10
\mathchardef\twoheadleftarrow="3\msx@11
\mathchardef\leftleftarrows="3\msx@12
\mathchardef\rightrightarrows="3\msx@13
\mathchardef\upuparrows="3\msx@14
\mathchardef\downdownarrows="3\msx@15
\mathchardef\upharpoonright="3\msx@16
\let\restriction=\upharpoonright
\mathchardef\downharpoonright="3\msx@17
\mathchardef\upharpoonleft="3\msx@18
\mathchardef\downharpoonleft="3\msx@19
\mathchardef\rightarrowtail="3\msx@1A
\mathchardef\leftarrowtail="3\msx@1B
\mathchardef\leftrightarrows="3\msx@1C
\mathchardef\rightleftarrows="3\msx@1D
\mathchardef\Lsh="3\msx@1E
\mathchardef\Rsh="3\msx@1F
\mathchardef\rightsquigarrow="3\msx@20
\mathchardef\leftrightsquigarrow="3\msx@21
\mathchardef\looparrowleft="3\msx@22
\mathchardef\looparrowright="3\msx@23
\mathchardef\circeq="3\msx@24
\mathchardef\succsim="3\msx@25
\mathchardef\gtrsim="3\msx@26
\mathchardef\gtrapprox="3\msx@27
\mathchardef\multimap="3\msx@28
\mathchardef\therefore="3\msx@29
\mathchardef\because="3\msx@2A
\mathchardef\doteqdot="3\msx@2B
\let\Doteq=\doteqdot
\mathchardef\triangleq="3\msx@2C
\mathchardef\precsim="3\msx@2D
\mathchardef\lesssim="3\msx@2E
\mathchardef\lessapprox="3\msx@2F
\mathchardef\eqslantless="3\msx@30
\mathchardef\eqslantgtr="3\msx@31
\mathchardef\curlyeqprec="3\msx@32
\mathchardef\curlyeqsucc="3\msx@33
\mathchardef\preccurlyeq="3\msx@34
\mathchardef\leqq="3\msx@35
\mathchardef\leqslant="3\msx@36
\mathchardef\lessgtr="3\msx@37
\mathchardef\backprime="0\msx@38
\mathchardef\risingdotseq="3\msx@3A
\mathchardef\fallingdotseq="3\msx@3B
\mathchardef\succcurlyeq="3\msx@3C
\mathchardef\geqq="3\msx@3D
\mathchardef\geqslant="3\msx@3E
\mathchardef\gtrless="3\msx@3F
\mathchardef\sqsubset="3\msx@40
\mathchardef\sqsupset="3\msx@41
\mathchardef\vartriangleright="3\msx@42
\mathchardef\vartriangleleft="3\msx@43
\mathchardef\trianglerighteq="3\msx@44
\mathchardef\trianglelefteq="3\msx@45
\mathchardef\bigstar="0\msx@46
\mathchardef\between="3\msx@47
\mathchardef\blacktriangledown="0\msx@48
\mathchardef\blacktriangleright="3\msx@49
\mathchardef\blacktriangleleft="3\msx@4A
\mathchardef\vartriangle="0\msx@4D
\mathchardef\blacktriangle="0\msx@4E
\mathchardef\triangledown="0\msx@4F
\mathchardef\eqcirc="3\msx@50
\mathchardef\lesseqgtr="3\msx@51
\mathchardef\gtreqless="3\msx@52
\mathchardef\lesseqqgtr="3\msx@53
\mathchardef\gtreqqless="3\msx@54
\mathchardef\Rrightarrow="3\msx@56
\mathchardef\Lleftarrow="3\msx@57
\mathchardef\veebar="2\msx@59
\mathchardef\barwedge="2\msx@5A
\mathchardef\doublebarwedge="2\msx@5B
\mathchardef\angle="0\msx@5C
\mathchardef\measuredangle="0\msx@5D
\mathchardef\sphericalangle="0\msx@5E
\mathchardef\varpropto="3\msx@5F
\mathchardef\smallsmile="3\msx@60
\mathchardef\smallfrown="3\msx@61
\mathchardef\Subset="3\msx@62
\mathchardef\Supset="3\msx@63
\mathchardef\Cup="2\msx@64
\let\doublecup=\Cup
\mathchardef\Cap="2\msx@65
\let\doublecap=\Cap
\mathchardef\curlywedge="2\msx@66
\mathchardef\curlyvee="2\msx@67
\mathchardef\leftthreetimes="2\msx@68
\mathchardef\rightthreetimes="2\msx@69
\mathchardef\subseteqq="3\msx@6A
\mathchardef\supseteqq="3\msx@6B
\mathchardef\bumpeq="3\msx@6C
\mathchardef\Bumpeq="3\msx@6D
\mathchardef\lll="3\msx@6E
\let\llless=\lll
\mathchardef\ggg="3\msx@6F
\let\gggtr=\ggg
\mathchardef\circledS="0\msx@73
\mathchardef\pitchfork="3\msx@74
\mathchardef\dotplus="2\msx@75
\mathchardef\backsim="3\msx@76
\mathchardef\backsimeq="3\msx@77
\mathchardef\complement="0\msx@7B
\mathchardef\intercal="2\msx@7C
\mathchardef\circledcirc="2\msx@7D
\mathchardef\circledast="2\msx@7E
\mathchardef\circleddash="2\msx@7F
\def\ulcorner{\delimiter"4\msx@70\msx@70 }
\def\urcorner{\delimiter"5\msx@71\msx@71 }
\def\llcorner{\delimiter"4\msx@78\msx@78 }
\def\lrcorner{\delimiter"5\msx@79\msx@79 }
\def\yen{\mathhexbox\msx@55 }
\def\checkmark{\mathhexbox\msx@58 }
\def\circledR{\mathhexbox\msx@72 }
\def\maltese{\mathhexbox\msx@7A }
\mathchardef\lvertneqq="3\msy@00
\mathchardef\gvertneqq="3\msy@01
\mathchardef\nleq="3\msy@02
\mathchardef\ngeq="3\msy@03
\mathchardef\nless="3\msy@04
\mathchardef\ngtr="3\msy@05
\mathchardef\nprec="3\msy@06
\mathchardef\nsucc="3\msy@07
\mathchardef\lneqq="3\msy@08
\mathchardef\gneqq="3\msy@09
\mathchardef\nleqslant="3\msy@0A
\mathchardef\ngeqslant="3\msy@0B
\mathchardef\lneq="3\msy@0C
\mathchardef\gneq="3\msy@0D
\mathchardef\npreceq="3\msy@0E
\mathchardef\nsucceq="3\msy@0F
\mathchardef\precnsim="3\msy@10
\mathchardef\succnsim="3\msy@11
\mathchardef\lnsim="3\msy@12
\mathchardef\gnsim="3\msy@13
\mathchardef\nleqq="3\msy@14
\mathchardef\ngeqq="3\msy@15
\mathchardef\precneqq="3\msy@16
\mathchardef\succneqq="3\msy@17
\mathchardef\precnapprox="3\msy@18
\mathchardef\succnapprox="3\msy@19
\mathchardef\lnapprox="3\msy@1A
\mathchardef\gnapprox="3\msy@1B
\mathchardef\nsim="3\msy@1C
%\mathchardef\napprox="3\msy@1D
\mathchardef\ncong="3\msy@1D
\def\napprox{\not\approx}
\mathchardef\varsubsetneq="3\msy@20
\mathchardef\varsupsetneq="3\msy@21
\mathchardef\nsubseteqq="3\msy@22
\mathchardef\nsupseteqq="3\msy@23
\mathchardef\subsetneqq="3\msy@24
\mathchardef\supsetneqq="3\msy@25
\mathchardef\varsubsetneqq="3\msy@26
\mathchardef\varsupsetneqq="3\msy@27
\mathchardef\subsetneq="3\msy@28
\mathchardef\supsetneq="3\msy@29
\mathchardef\nsubseteq="3\msy@2A
\mathchardef\nsupseteq="3\msy@2B
\mathchardef\nparallel="3\msy@2C
\mathchardef\nmid="3\msy@2D
\mathchardef\nshortmid="3\msy@2E
\mathchardef\nshortparallel="3\msy@2F
\mathchardef\nvdash="3\msy@30
\mathchardef\nVdash="3\msy@31
\mathchardef\nvDash="3\msy@32
\mathchardef\nVDash="3\msy@33
\mathchardef\ntrianglerighteq="3\msy@34
\mathchardef\ntrianglelefteq="3\msy@35
\mathchardef\ntriangleleft="3\msy@36
\mathchardef\ntriangleright="3\msy@37
\mathchardef\nleftarrow="3\msy@38
\mathchardef\nrightarrow="3\msy@39
\mathchardef\nLeftarrow="3\msy@3A
\mathchardef\nRightarrow="3\msy@3B
\mathchardef\nLeftrightarrow="3\msy@3C
\mathchardef\nleftrightarrow="3\msy@3D
\mathchardef\divideontimes="2\msy@3E
\mathchardef\varnothing="0\msy@3F
\mathchardef\nexists="0\msy@40
\mathchardef\mho="0\msy@66
\mathchardef\eth="0\msy@67
\mathchardef\eqsim="3\msy@68
\mathchardef\beth="0\msy@69
\mathchardef\gimel="0\msy@6A
\mathchardef\daleth="0\msy@6B
\mathchardef\lessdot="3\msy@6C
\mathchardef\gtrdot="3\msy@6D
\mathchardef\ltimes="2\msy@6E
\mathchardef\rtimes="2\msy@6F
\mathchardef\shortmid="3\msy@70
\mathchardef\shortparallel="3\msy@71
\mathchardef\smallsetminus="2\msy@72
\mathchardef\thicksim="3\msy@73
\mathchardef\thickapprox="3\msy@74
\mathchardef\approxeq="3\msy@75
\mathchardef\succapprox="3\msy@76
\mathchardef\precapprox="3\msy@77
\mathchardef\curvearrowleft="3\msy@78
\mathchardef\curvearrowright="3\msy@79
\mathchardef\digamma="0\msy@7A
\mathchardef\varkappa="0\msy@7B
\mathchardef\hslash="0\msy@7D
\mathchardef\hbar="0\msy@7E
\mathchardef\backepsilon="3\msy@7F
% Use the next 4 lines with AMS-TeX:
%\def\Bbb{\relaxnext@\ifmmode\let\next\Bbb@\else
% \def\next{\Err@{Use \string\Bbb\space only in math mode}}\fi\next}
%\def\Bbb@#1{{\Bbb@@{#1}}}
%\def\Bbb@@#1{\noaccents@\fam\msyfam#1}
% Use the next 4 lines if NOT using AMS-TeX:
\def\Bbb{\ifmmode\let\next\Bbb@\else
 \def\next{\errmessage{Use \string\Bbb\space only in math mode}}\fi\next}
\def\Bbb@#1{{\Bbb@@{#1}}}
\def\Bbb@@#1{\fam\msyfam#1}

\catcode`\@=12

